An online adaptive finite-element method for nonsmooth PDE-constrained optimization

We present a trust-region-based adaptive finite-element algorithm for numerically solving a class of nonsmooth PDE-constrained optimization problems that includes problems with sparsifying regularizers and convex constraints. In particular, we consider the class of problems whose objective function is the sum of a smooth, possibly nonconvex, function and a nonsmooth extended real-valued convex function. Our method combines the robustness of inexact trust-region algorithms for nonsmooth problems with the efficiency of adaptive finite-element discretizations. Starting from a coarse mesh, the algorithm automatically refines the discretization based on reliable a posteriori error estimators for both the state and adjoint equations, systematically controlling the accuracy of the computed smooth objective function value and gradient. This adaptivity mechanism balances computational cost and solution accuracy, enabling high resolution of localized phenomena and sparsity structures in the state and control variables. We demonstrate the performance of our algorithm through numerical experiments on representative control and topology optimization examples.

==> conclusions.tex <==
We have introduced an adaptive finite-element trust-region algorithm for
solving PDE-constrained optimization problems based on \cite{MR4620236} to control
objective function and gradient error. We quantify the latter via a {\it reliable  a
posteriori error estimators} for the state and adjoint equations.  
We demonstrated the performance of our method on
a Poisson problem in a nonconvex domain and two variations
of a density-based topology optimization problem.
Future work entails implementation of both refinement and coarsening, the latter of which
entails removing elements until our error indicators violate the perscribed tolerance. 
We also can implement $r$- or $p$-adaptivity,
as well as compare against other algorithms, e.g. goal-oriented adaptivity \cite{besier2012qoi},
and finite element discretizations \cite{mfem}.


